Differential Privacy of Aggregated DC Optimal Power Flow Data

We consider the problem of privately releasing aggregated network statistics obtained from solving a DC optimal power flow (OPF) problem. It is shown that the mechanism that determines the noise distribution parameters are linked to the topology of the power system and the monotonicity of the network. We derive a measure of "almost" monotonicity and show how it can be used in conjunction with a linear program in order to release aggregated OPF data using the differential privacy framework.

==> Privacy.tex <==
\section{Differential Privacy}

\subsection{OPF Data Privacy}
Ideally both the generations $\sgen$ and loads $\sload$ are  available 
for the research community to build realistic power system models from.
However, load data may contain sensitive information, and hence it is desirable 
to preserve the privacy of $\sload$.

Suppose $\query(\sgen,\sload)$ is a (randomized) function of $(\sgen,\sload)$, and acts as the mechanism of the data. %\ja{[I don't think system is the right word here]}. 
It is reasonable to assume that $\sgen$ is always chosen as the
unique optimal solution to the OPF problem, i.e., $\sgen=\OPF(\sload)$.
Then we can write $\query(\sgen,\sload)$ as $\query(\OPF(\sload),\sload)$.
The privacy problem is to design a mechanism that hides individual load 
changes
when the database $\data$ containing the vectors $\sgen, \sload$ is queried. 
We let  $\Delta$ denote the changes to an individual load, 
i.e.,  $\sload_i \leftarrow \sload_i \pm\Delta$ for some  $\Delta>0$.
To address this problem, we introduce a modified version of differential privacy: 
%we then define the \ja{power system $(\Delta,\varrho)$-differential privacy by modifying Definition \ref{Df:DP}.}
\begin{definition}
For $\Delta,\varrho>0$, the mechanism $\query$ preserves $(\Delta,\varrho)$-differential privacy if and only if $\forall (\sload)',(\sload)''$ such that $\|(\sload)'-(\sload)''\|_0\leq1$ and $\|(\sload)'-(\sload)''\|_1\leq\Delta$, 
and $\forall \W\subseteq\Real^r$, we have
\begin{align*}
\nonumber
&\Prob\{\query(\OPF((\sload)'),(\sload)')\in\W\}\\
\leq &\exp(\varrho)\cdot\Prob\{\query(\OPF((\sload)''),(\sload)'')\in\W\}.
\end{align*}
\end{definition}

Theorem~\ref{thm:lapDP} can be readily extended to our $(\Delta,\varrho)$-differential privacy.
\begin{lemma}\label{lm:dp}
Suppose  $\tilde{\query}(\sgen,\sload)$ is a deterministic function of $(\sgen,\sload)$ satisfying that
$\forall (\sload)',(\sload)''$ such that $\|(\sload)'-(\sload)''\|_0\leq1$ and $\|(\sload)'-(\sload)''\|_1\leq\Delta$, 
we have 
\begin{align*}%\label{eq:sensitivity}
\|\tilde{\query}(\OPF((\sload)'),(\sload)')-\tilde{\query}(\OPF((\sload)''),(\sload)'')\|_1\leq \Delta_1.
\end{align*}
Then the mechanism $\query=\tilde{\query}+\dpnoises$, where all $Y_i$ are drawn 
from independent Laplace distributions $\Lap(\Delta_1/\varrho)$,
 preserves $(\Delta,\varrho)-$differential privacy.
\end{lemma}
%The left hand side of \eqref{eq:sensitivity} is also known as the $L_1$-sensitivity, 
%and Lemma \ref{lm:dp} shows that a good estimation of \eqref{eq:sensitivity} can potentially help design the suitable noise level in order to preserve the differential privacy.

In the next section, we will introduce the \emph{aggregation mechanism} as an example 
for estimating the $L_1$-sensitivity.%, where 
%$\tilde{\query}$ is the vector of regional sums of the injections. \ja{[Too vague - rewrite...]}
%\fz{power injections $\sgen$ and $\sload$ are geographically aggregated, and $\tilde{\query}$ is the vector of the aggregated data for each region.[Another way is to simply delete the second half of the last sentence as the detailed definition will be immediately available in the next section.]}


